Telepresence Video Quality Assessment

Video conferencing, which includes both video and audio content, has contributed to dramatic increases in Internet traffic, as the COVID-19 pandemic forced millions of people to work and learn from home. Global Internet traffic of video conferencing has dramatically increased Because of this, efficient and accurate video quality tools are needed to monitor and perceptually optimize telepresence traffic streamed via Zoom, Webex, Meet, etc. However, existing models are limited in their prediction capabilities on multi-modal, live streaming telepresence content. Here we address the significant challenges of Telepresence Video Quality Assessment (TVQA) in several ways. First, we mitigated the dearth of subjectively labeled data by collecting ~2k telepresence videos from different countries, on which we crowdsourced ~80k subjective quality labels. Using this new resource, we created a first-of-a-kind online video quality prediction framework for live streaming, using a multi-modal learning framework with separate pathways to compute visual and audio quality predictions. Our all-in-one model is able to provide accurate quality predictions at the patch, frame, clip, and audiovisual levels. Our model achieves state-of-the-art performance on both existing quality databases and our new TVQA database, at a considerably lower computational expense, making it an attractive solution for mobile and embedded systems.

==> algo_online_predict.tex <==
% \tcp*{this is another comment}
% \tcc{this is another comment}
\begin{algorithm}[H]
\DontPrintSemicolon
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
  \KwInput{
    Live video stream ($V$), 
    % Feature extractors, regressors
    Sampling window ($T$),
    Clip size ($N$)
  }
  \KwOutput{Path level predictions $\{ s_t^{(p_i)}  \}$, \\
\Indp \Indp Frame level predictions $s^{(f)}_{t}$, \\
Clip level predictions, $s^{(v)}_{t}$, \\
Audiovisual level predictions $s^{(av)}_{t}$ }
%   \KwData{Testing set $x$}
  Initialize a queue $Q$ to queue $N$ incoming frames;
  $t \gets 1$ \\
  $\textbf{h}^{(v)}_0, \textbf{h}^{(a)}_0 \gets \textbf{0},  \textbf{0}$ % all 0s \Comment{This is a comment}
  
   \While{ new frames available from $V$ } %  != \emptyset
   { 
        Add frame $f_t$ from $V$ to $Q$ \\
   		\If{$t~ \% ~T$} {
   		    Fetch a frame $f_i$, a video clip $c_i$ from $Q$\\
   		    % Extract IQA features 
   		    $\textbf{x}^{(f)}_{t}  \gets \text{MobileNetV3}( f_t )$ \\
   		    $\textbf{x}^{(c)}_{t}  \gets \text{MobileNetV2}^{3d}( c_t )$ \\
   		    $\textbf{x}^{(c)}_{t} \gets \textbf{x}^{(f)}_{t} \oplus \textbf{x}^{(c)}_{t} $ \\
   		   $s^{(v)}_{t}  \gets \textbf{r}^{(a)} ( \textbf{x}^{(v)}_{t} , \textbf{h}^{(v)}_t )$
   		   % $s^{(v)}_i = \text{TeleVQA-V}( f_i, c_i )$ \\
   		   % $s^{(a)}_i = \text{TeleVQA-A}( a_i )$ \\
   		   % $f_(a) = f_(p_i) \oplus f_(f_i) \oplus f_(c_i)$\\
   		   % $s^{(c)}_{t}, h_{t} \gets \textbf{r}^{(v)} ( f, h_{t-1}) $\\
   		   
   		   
   		 \If{audio clip $a_i$ is available}
   		{
   		$\textbf{x}^{(a)}_{t}  \gets \text{YAMNet}(  \text{STFT}(a_t) )$ \\
        $s^{(a)}_{t}  \gets \textbf{r}^{(a)} ( \textbf{x}^{(a)}_{t} , \textbf{h}^{(a)}_t )$
        }
        \Else{$s^{(a)}_{t} \gets s^{(a)}_{t-1}$}
   		
   		}
   		$s^{(av)}_{t} \gets s^{(a)}_{t} \otimes s^{(v)}_{t} $ \\
   		$t \gets t + 1$
   }

\caption{Online multimodal quality prediction}
\end{algorithm}

% \begin{algorithm}
% \caption{Online multimodal quality prediction}\label{alg:cap}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \begin{algorithmic}
% % (x_i, y_i, h_i, w_i)
% \Require 
% % $\{ (x_i, y_i, h_i, w_i) \}, f_t, c_t, a_t$
% \Ensure 
% % $\{ s_t^{(p_i)}  \}, s^{(f)}_{t}, s^{(f)}_{t}, s^{(c)}_{t}, s^{(a)}_{t}$ 
% \State 
% % new frames & audio clip available from $V$

% \While {$t~ \% ~T$}
% % \State Add frame $f_i$ from V to queue Q;
% % \If{$i ~~\% ~~T$}
% \State 
% % , and an audio clip $a_i$
% \State $N \gets \frac{N}{2}$  
% % \ElsIf{$N$ is odd}
% \State $f_(a) = f_(p_i) \oplus f_(f_i) \oplus f_(c_i)$
% \State 

% \State 
% \State $t \gets t + 1$
% % \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

==> tbl/_iqa_old.tex <==
\begin{table}[b]
% \captionsetup{font=scriptsize}
% \setlength\extrarowheight{1.0pt}
\centering
\footnotesize
% \vspace{0.8em}
\begin{tabular}{P{3.1cm}|P{0.85cm}|P{0.85cm}|P{0.85cm}|P{0.85cm}}
\hline
& \multicolumn{2}{c|}{\textbf{LIVE-FB}} & \multicolumn{2}{c}{\textbf{LIVE-FB-Large}} \\
\hline
\textbf{Model} & \textbf{SRCC} & \textbf{LCC} & \textbf{SRCC} & \textbf{LCC} \\
\hline
NIQE \cite{niqe} & 0.094 & 0.131 & 0.211 & 0.288 \\
BRISQUE \cite{brisque} & 0.303 & 0.341 & 0.288 & 0.373 \\
\hline
CNNIQA \cite{cnnIqa} & 0.259 & 0.242 & 0.266 & 0.223 \\
NIMA \cite{nima} & 0.521 & 0.609 & 0.583 & 0.639 \\
\hline
% P2P-BM ~\cite{paq2piq} & 0.525 & 0.599 & 0.571 & 0.623 \\
% P2P-RM  & 0.541	& 0.618 & 0.576 & 0.655 \\
P2P-FM ~\cite{paq2piq} & {0.562}	& {0.649} & {0.601} & \textbf{0.685} \\
TeleVQA   & \textbf{0.580} & \textbf{0.675} 
& \textbf{0.619}	& {0.677}\\
\hline
\end{tabular}
\vspace{0.5em}
\caption{\footnotesize{\textbf{Picture quality predictions: }
Performance of picture quality models on the full-size validation and test pictures in the LIVE-FB database. A higher value indicates superior performance. NIQE is not trained. \vspace{-0.5em}}}
\vspace{-1.5em}
\label{tbl:onFlive}
\end{table}


\begin{figure}[b!]
\centering
\includegraphics[width=0.5\textwidth]{images/5_roipool.png}
\caption{Our model predicts a more accurate patch quality map.}
\vspace{-1em}
\label{fig:runtime}
\end{figure}


%%% table  CLIVE and KONIQ
\begin{table}[t]
% \captionsetup{font=scriptsize}
% \setlength\extrarowheight{1.0pt}
\centering
\footnotesize
% \vspace{0.8em}
\begin{tabular}{P{3.1cm}||P{0.7cm}|P{0.7cm}||P{0.7cm}|P{0.7cm}}
% \hline
% & \multicolumn{4}{c}{\textbf{Validation Set}} \\
\hline
& \multicolumn{2}{c||}{\textbf{CLIVE} \cite{clive}} & \multicolumn{2}{c}{\textbf{KonIQ} \cite{koniq}} \\
\hline
\textbf{Model} & \textbf{SRCC} & \textbf{LCC} & \textbf{SRCC} & \textbf{LCC} \\
\hline
NIQE \cite{niqe} & 0.503 & 0.528 & 0.534 & 0.509 \\
BRISQUE \cite{brisque} & 0.660 & 0.621 & 0.641 & 0.596 \\
\hline
CNNIQA \cite{cnnIqa} & 0.559 & 0.459 & 0.596	& 0.403 \\
NIMA \cite{nima} & 0.712 & 0.705 & 0.666	& 0.721 \\
\hline
P2P-FM~\cite{paq2piq} & 0.784	& 0.754 & \textbf{0.788}	& \textbf{0.808} \\
TeleVQA & \textbf{0.788}	& \textbf{0.813} & {0.772}	& {0.800} \\
\hline 
%\hline
%\textit{Best model} \cite{mixedDBiqa} &	0.851 & & 0.894 & \\
% \hline
\end{tabular}
\vspace{0.5em}
\caption{\footnotesize{\textbf{Cross-database comparisons:} Results when models trained on the LIVE-FB database are applied on CLIVE \cite{clive} and KonIQ \cite{koniq} \textbf{without fine-tuning.}
% \vspace{-1.2em}
}}
% \vspace{-1.5em}
\label{tbl:cliveKoniq}
\end{table}

==> tbl/databases_v1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
% \captionsetup{font=scriptsize}
\vspace{-0.1in}
\scriptsize
\centering
\begin{tabular}{@{}cllllrrrrrrrrccc@{}}
\toprule







Year & Name         & Focus        & Video                                  & Audio                 & \# Unique contents & \# Total videos & Distortion Type             & Methodology    & \# Annotators & \# Total Ratings \\ \midrule
2010 & PLYM         & Mobile IP    & 144 p, 8–15 fps, 7–14 s                & 16-bits, 8 kHz        & 6                  & 60              & C,T & ACR            & 16            & 960              \\
2012 & VQEG-MM      & IPTV         & 480 p, 30 fps, 10 s                    & 16-bits, 48 kHz       & 10                 & 60              & C                 & ACR            & 35            & 2100             \\
2012 & TUM          & IPTV         & 1080 p, 50 fps, 10 s                   & -                     & 5                  & 20              & C,T & ACR (11-point) & 21            & 420              \\
2013 & UnB-AVQ 2013 & IPTV         & 720 p, 4:2:0, 30 fps                   & 16-bit, 48 kHz, 8 s   & 8                  & 72              & C                 & ACR            & 16            & 1, 152           \\
2016 & INRS         & IPTV         & 720 p, 42 s                            & -                     & 1                  & 160             & C,T & ACR            & 30            & 4, 800           \\
2016 & MMSPG        & IPTV         & 2160-1080-720 p, 24 fps                & Stereo, 5.1 Surround  & 9                  & 27              & Display devices             & ACR{[}1–9{]}   & 20            & 540              \\
2018 & UnB-AVQ 2018 & IPTV         & 720 p, 30 fps, 4:2:0                   & 16-bits, 48 kHz, 37 s & 60                 & 720             & C,T & Immersive      & 60            & 43, 200          \\
2018 & UnB-AVQ 2018 & IPTV         & 720 p, 30 fps, 4:2:0                   & 16-bits, 48 kHz, 35 s & 40                 & 800             & C,T & Immersive      & 40            & 32, 000          \\
2018 & UnB-AVQ 2018 & IPTV         & 720 p, 30 fps, 4:2:0                   & 16-bits, 48 kHz, 34 s & 40                 & 800             & C,T & Immersive      & 40            & 32, 000          \\
2018 & LIVE-NFLX-II & IPTV         & 1080 p, 30 fps, 25 s                   & -                     & 15                 & 420             & C,T & ACR{[}1–100{]} & 65            & 27, 300          \\
2020 & LIVE-SJTU    & IPTV         & 1080 p, 30 fps, 8 s                    & 16-bits, 48 kHz       & 14                 & 336             & C                 & ACR            & 35            & 11, 760          \\
2021 & Ours         & telepresence & $<$ 1080p, 10-60 fps, 5-15 s & 16-bits, 48 kHz       & 2320               & 2320            & In-the-wild                 & SSCQS          & 526           & \textbf{78, 880} \\ \bottomrule
\end{tabular}
\end{table*}









% Year & Name         & Focus     & Video                   & Audio                 & SRC & HRC & TS  & \# Distortion                                    & Methodology & Scale       & MOS   & n   &  &  &  \\ \midrule
% 2010 & PLYM         & Mobile IP &                         &                       &     &     &     &                                                  &             &             &       &     &  &  &  \\
% 2012 & VQEG-MM      & IPTV      & 480 p, 30 fps, 10 s     & 48 kHz, 16-bits       & 10  & 5   & 60  & AC, VC                                           & ACR         & {[}1–5{]}   & MOSav & 35  &  &  &  \\
% 2012 & TUM          & IPTV      & 1080 p, 50 fps, 10 s    & -                     & 5   & 4   & 20  & VC, TE                                           & ACR         & 11-point    & MOSav & 21  &  &  &  \\
% 2013 & UnB-AVQ 2013 & IPTV      & 720 p, 4:2:0, 30 fps    & 16-bit, 48 kHz, 8 s   & 8   & 12  & 72  & AC: MPEG-1 Layer 3  VC:H.264                     & ACR         & {[}1–5{]}   & MOSav & 16  &  &  &  \\
% 2016 & INRS         & IPTV      & 720 p, 42 s             & -                     & 1   & 160 & 160 & VC: H.264, TE                                    & ACR         & {[}1–5{]}   & MOSav & 30  &  &  &  \\
% 2016 & MMSPG        & IPTV      & 2160-1080-720 p, 24 fps & Stereo, 5.1 Surround  & 9   & 3   & 27  & Display devices                                  & ACR         & {[}1–9{]}   & MOSav & 20  &  &  &  \\
% 2018 & UnB-AVQ 2018 & IPTV      & 720 p, 30 fps, 4:2:0    & 16-bits, 48 kHz, 37 s & 60  & 12  & 720 & VC: H.264–H.265, TE, FF                          & Immersive   & {[}1–5{]}   & MOSav & 60n &  &  &  \\
% 2018 & UnB-AVQ 2018 & IPTV      & 720 p, 30 fps, 4:2:0    & 16-bits, 48 kHz, 35 s & 40  & 20  & 800 & Ch, Cl, CS, Ec, BG Noise                         & Immersive   & {[}1–5{]}   & MOSav & 40  &  &  &  \\
% 2018 & UnB-AVQ 2018 & IPTV      & 720 p, 30 fps, 4:2:0    & 16-bits, 48 kHz, 34 s & 40  & 20  & 800 & Ch, Cl, CS, Ec, BG Noise VC: H.264–H.265, TE, FF & Immersive   & {[}1–5{]}   & MOSav & 40  &  &  &  \\
% 2018 & LIVE-NFLX-II & IPTV      & 1080 p, 30 fps, 25 s    & -                     & 15  & 28  & 420 & TE, BA                                           & ACR         & {[}1–100{]} & MOSav & 65  &  &  &  \\
% 2020 & LIVE-SJTU    & IPTV      & 1080 p, 30 fps, 8 s     & 16-bits, 48 kHz       & 14  & 24  & 336 & VC: H.265, Scaling AC:AAC                        & ACR         & {[}1–5{]}   & MOSav & 35  &  &  &  \\ \bottomrule


==> tbl/databases_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t!]

% \vspace{-0.1in}
\caption{\textbf{Summary of Popular Audiovisual QA Databases}. VC: Video compression; TE: Transmission Errors; AC: Audio compression;
% ``In-the-wild'' databases contain videos impaired by complex mixtures of highly diverse distortions, each as unique as the videos they afflict.
}
\scriptsize
\centering
\begin{tabular}{@{}cllrrccrr@{}}
\toprule
Year & Name         & Focus        & \# Unique contents & \# Total videos & Distortion Type             & Methodology    & \# Annotators & \# Total Ratings \\ \midrule
2010 & PLYM~\cite{PLYM}         & Mobile IP    & 6                  & 60              & Synthetic (VC, TE) & ACR            & 16            & 960              \\
2012 & VQEG-MM~\cite{VQEG_MM}      & IPTV         & 10                 & 60              & Synthetic (VC, AC)                 & ACR            & 35            & 2100             \\
2012 & TUM~\cite{tum1080p}          & IPTV         & 5                  & 20              & Synthetic (VC, TE) & ACR (11-point) & 21            & 420              \\
2013 & UnB-AVQ 2013~\cite{UnB2013} & IPTV         & 8                  & 72              & Synthetic (VC, AC)                 & ACR            & 16            & 1, 152           \\
2016 & INRS~\cite{INRS, INRS2}         & IPTV         & 1                  & 160             & Synthetic (VC, TE) & ACR            & 30            & 4, 800           \\
2016 & MMSPG~\cite{MMSPG}        & IPTV         & 9                  & 27              & Display devices             & ACR{[}1–9{]}   & 20            & 540              \\
2018 & UnB-AVQ 2018 Exp1~\cite{UnB2018} & IPTV         & 60                 & 720             & Synthetic (VC, TE) & Immersive      & 60            & 43, 200          \\
2018 & UnB-AVQ 2018 Exp2~\cite{UnB2018} & IPTV         & 40                 & 800             & Synthetic (VC, TE) & Immersive      & 40            & 32, 000          \\
2018 & UnB-AVQ 2018 Exp3~\cite{UnB2018} & IPTV         & 40                 & 800             & Synthetic (VC, TE) & Immersive      & 40            & 32, 000          \\
2018 & LIVE-NFLX-II~\cite{LIVE_NFLIX2} & IPTV         & 15                 & 420             & Synthetic (TE) & ACR{[}1–100{]} & 65            & 27, 300          \\
2020 & LIVE-SJTU~\cite{min2020study}    & IPTV         & 14                 & 336             & Synthetic (VC, AC)                 & ACR            & 35            & 11, 760          \\
\textbf{2021} & \textbf{Proposed database}         & \textbf{Telepresence} & \textbf{2320}               & \textbf{2320}            & \textbf{In-the-wild}                 & \textbf{SSCQS}          & \textbf{526}           & \textbf{78, 880} \\ \bottomrule
\end{tabular}
\vspace{-1em}
\label{tab:databases_summary}
\end{table*}

==> tbl/iqa.tex <==
\begin{table*}[tb]
\caption{\footnotesize{\textbf{Picture quality predictions: }
Performance of picture quality models on different databases~\cite{paq2piq}. A higher value indicates superior performance. NIQE is not a trained model. \deepti{Need models that are not from LIVE lab evaluated and reported.}}}
\vspace{0.3em}
% \captionsetup{font=scriptsize}
% \setlength\extrarowheight{1.0pt}
\centering
\footnotesize
% \vspace{0.8em}
\begin{tabular}
% {P{3.1cm}|P{0.71cm}|P{0.71cm}|P{0.71cm}|P{0.71cm}}
{l||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
}
\hline
& \multicolumn{2}{c||}{\textbf{LIVE-FB~\cite{paq2piq} }} 
& \multicolumn{2}{c||}{\textbf{LIVE-FB-Patch 1 }}  
& \multicolumn{2}{c||}{\textbf{LIVE-FB-Patch 2 }} 
& \multicolumn{2}{c||}{\textbf{LIVE-FB-Patch 3 }} 
& \multicolumn{2}{c||}{\textbf{CLIVE~\cite{clive} }} 
& \multicolumn{2}{c}{\textbf{KonIQ~\cite{koniq} }} 
\\
\hline
\textbf{Model} 
  & \textbf{SRCC} & \textbf{LCC} 
  & \textbf{SRCC} & \textbf{LCC} 
  & \textbf{SRCC} & \textbf{LCC}  
  & \textbf{SRCC} & \textbf{LCC}  
  & \textbf{SRCC} & \textbf{LCC} 
  & \textbf{SRCC} & \textbf{LCC} \\
\hline
NIQE \cite{niqe} & 0.094 & 0.131 & 0.503 & 0.528 & 0.109 & 0.106 & 0.029 & 0.011 & 0.052 & 0.154 & 0.534 & 0.509 \\
BRISQUE \cite{brisque} & 0.303 & 0.341 & 0.660 & 0.621 & 0.384 & 0.467 & 0.442 & 0.503 & 0.495 & 0.494 & 0.641 & 0.596\\
\hline
CNNIQA \cite{cnnIqa} & 0.259 & 0.242 & 0.559 & 0.459 & 0.438 & 0.400 & 0.522 & 0.449 & 0.580 & 0.481 & 0.596	& 0.403\\
NIMA \cite{nima} & 0.521 & 0.609 & 0.712 & 0.705 & 0.587 & 0.637 & 0.547 & 0.560 & 0.395 & 0.411 & 0.666	& 0.721 \\
\hline
% P2P-BM ~\cite{paq2piq} & 0.525 & 0.599 & 0.571 & 0.623 \\
% P2P-RM  & 0.541	& 0.618 & 0.576 & 0.655 \\
P2P-FM ~\cite{paq2piq} & {0.562}	& {0.649} & {0.784} & {0.754} & 0.658 & 0.744 & 0.698 & 0.762 & 0.756 & 0.783 & \textbf{0.788} & \textbf{0.808} \\
\textbf{Tele-VQA}   & \textbf{0.580} & \textbf{0.675}  
& \textbf{0.788}	& \textbf{0.813}  & \textbf{0.676} & \textbf{0.769} & \textbf{0.725} & \textbf{0.783} & \textbf{0.767} & \textbf{0.795} & {0.772}	& {0.800}\\
\hline
\end{tabular}
\vspace{-1em}
\label{tbl:onFlive}
\end{table*}



==> tbl/iqa_cross.tex <==
\begin{table*}[tb]
\caption{\footnotesize{\textbf{Picture quality predictions: }
Performance of picture quality models on different databases~\cite{paq2piq}. A higher value indicates superior performance. 
}}

% \deepti{Need models that are not from LIVE lab evaluated and reported.}Thanks, Fixed
\vspace{0.3em}
% \captionsetup{font=scriptsize}
% \setlength\extrarowheight{1.0pt}
\centering
% \footnotesize
\scriptsize
% \vspace{0.8em}
\begin{tabular}
% {P{3.1cm}|P{0.71cm}|P{0.71cm}|P{0.71cm}|P{0.71cm}}
{l
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
||P{0.71cm}|P{0.71cm}
}
\hline
& \multicolumn{2}{c||}{\textbf{LIVE-FB-Patch 1 }}  
& \multicolumn{2}{c||}{\textbf{LIVE-FB-Patch 2 }} 
& \multicolumn{2}{c||}{\textbf{LIVE-FB-Patch 3 }} 
& \multicolumn{2}{c||}{\textbf{CLIVE~\cite{clive} }} 
& \multicolumn{2}{c}{\textbf{KonIQ~\cite{koniq} }} 
\\
\hline
\textbf{Model} 
  & \textbf{SRCC} & \textbf{LCC} 
  & \textbf{SRCC} & \textbf{LCC}  
  & \textbf{SRCC} & \textbf{LCC}  
  & \textbf{SRCC} & \textbf{LCC} 
  & \textbf{SRCC} & \textbf{LCC} 
\\
\hline
NIQE \cite{niqe} & 0.503 & 0.528 & 0.109 & 0.106 & 0.029 & 0.011 & 0.052 & 0.154 & 0.534 & 0.509 \\
BRISQUE \cite{brisque}  & 0.660 & 0.621 & 0.384 & 0.467 & 0.442 & 0.503 & 0.495 & 0.494 & 0.641 & 0.596\\
\hline
CNNIQA \cite{cnnIqa}  & 0.559 & 0.459 & 0.438 & 0.400 & 0.522 & 0.449 & 0.580 & 0.481 & 0.596	& 0.403\\
NIMA \cite{nima} &  0.712 & 0.705 & 0.587 & 0.637 & 0.547 & 0.560 & 0.395 & 0.411 & 0.666	& 0.721 \\
\hline
% P2P-BM ~\cite{paq2piq} & 0.525 & 0.599 & 0.571 & 0.623 \\
% P2P-RM  & 0.541	& 0.618 & 0.576 & 0.655 \\
P2P-FM ~\cite{paq2piq}  & {0.784} & {0.754} & 0.658 & 0.744 & 0.698 & 0.762 & 0.756 & 0.783 & \textbf{0.788} & \textbf{0.808} \\
\textbf{Tele-IQA}     
& \textbf{0.788}	& \textbf{0.813}  & \textbf{0.676} & \textbf{0.769} & \textbf{0.725} & \textbf{0.783} & \textbf{0.767} & \textbf{0.795} & {0.772}	& {0.800}\\
\hline
\end{tabular}
\vspace{-1.5em}
\label{tbl:onFlive}
\end{table*}


